Clustering is semidefinitely not that hard: Nonnegative SDP for manifold disentangling

In solving hard computational problems, semidefinite program (SDP) relaxations often play an important role because they come with a guarantee of optimality. Here, we focus on a popular semidefinite relaxation of K-means clustering which yields the same solution as the non-convex original formulation for well segregated datasets. We report an unexpected finding: when data contains (greater than zero-dimensional) manifolds, the SDP solution captures such geometrical structures. Unlike traditional manifold embedding techniques, our approach does not rely on manually defining a kernel but rather enforces locality via a nonnegativity constraint. We thus call our approach NOnnegative MAnifold Disentangling, or NOMAD. To build an intuitive understanding of its manifold learning capabilities, we develop a theoretical analysis of NOMAD on idealized datasets. While NOMAD is convex and the globally optimal solution can be found by generic SDP solvers with polynomial time complexity, they are too slow for modern datasets. To address this problem, we analyze a non-convex heuristic and present a new, convex and yet efficient, algorithm, based on the conditional gradient method. Our results render NOMAD a versatile, understandable, and powerful tool for manifold learning.

==> Clustering is semidefinitely not that hard/appendices.tex <==
\appendix

\section{Relationship with $K$-means}
\label{sec:kmeans}

$K$-means seeks to cluster a dataset $\set{X} = \{ \vect{x}_i \}_{i=1}^{n}$ by computing
\begin{equation}
	\tag{$K$-means}
	%
	\min_{\bm{\set{C}}_K}
	\sum_{k=1}^{K} \sum_{\vect{x}_i \in \set{C}_k}
	\norm{\vect{x}_i - \tfrac{1}{|\set{C}_k|} \sum_{\vect{x}_j \in \set{C}_k} \vect{x}_j }{2}^2 ,
	%
	\label[problem]{eq:kmeans}
\end{equation}
where $\bm{\set{C}}_K = \{ \set{C}_k\}_{k=1}^{K}$ is a partition of $\set{X}$, i.e., $\set{C}_{k} \cap \set{C}_{k'} = \emptyset$ and  $\bigcup_k \set{C}_k = \set{X}$.
Albeit its popularity, it is known to be NP-Hard and, in practice, users employ an heuristic \citep[][originally developed in 1957]{Lloyd1982} to find a solution.
The objective function of K-means, henceforth denoted $J_K$, can be rewritten (dropping the  terms that are constant with respect to $\set{C}_k$) as
\begin{equation}
	J_K = 
	- \sum_{k=1}^{K}
	\tfrac{1}{|\set{C}_k|} \sum_{\vect{x}_i, \vect{x}_j \in \set{C}_k} \transpose{\vect{x}}_i \vect{x}_j .
\end{equation}

Let $\mat{X} \in \Real^{d \times n}$ be the matrix formed by horizontally concatenating the vectors in $\set{X}$.
Let $\vect{z}_k \in \{ 0, 1 \}^{n}$ be the indicator vector of set $\set{C}_k$.
Let $\mat{Y}$ be the $k \times n$ matrix with rows $\vect{Y}_{k:} = |\set{C}_k|^{-1/2} \vect{z}_k$. We have
\begin{subequations}
\begin{align}
	J_K 
	&= - \sum_{k=1}^{K} \tfrac{1}{|\set{C}_k|} \sum_{i, j} \transpose{\vect{x}}_i \vect{x}_j \cdot (\transpose{\vect{z}}_k \vect{z}_k)_{ij} \\
	&= - \sum_{i, j} (\transpose{\mat{X}} \mat{X})_{ij} (\transpose{\mat{Y}} \mat{Y})_{ij} \\
	&= - \traceone{\transpose{\mat{X}} \mat{X} \transpose{\mat{Y}} \mat{Y}} .
	\label{eq:trace_xtxyty}
\end{align}
\end{subequations}

By construction, the matrix $\mat{Q} = \transpose{\mat{Y}} \mat{Y}$ exhibits the following properties
\begin{align}
%	\mat{Q} \in \set{V}_{\mat{Q}}^{n \times n} ,\quad
	\mat{Q} \vect{1} &= \vect{1} , \\
	\traceone{\mat{Q}} &= K .
\end{align}

Let $\mat{D}$ be the Gramian matrix, i.e., $\mat{D} = \transpose{\mat{X}} \mat{X}$.
We can then re-cast $K$-means as the optimization problem
\begin{equation}
	\max_{\mat{Y} \in \set{V}_{\mat{Y}}^{k \times n}}
	\traceone{\mat{D} \mat{Q}}
	%
	\quad\text{s.t.}\quad
	%
	\begin{aligned}
		& \mat{Q} \vect{1} = \vect{1} , \\
		& \traceone{\mat{Q}} = K , \\
		& \mat{Q} = \transpose{\mat{Y}} \mat{Y} .
	\end{aligned}
	\label[problem]{eq:kmeans_qyyt}
\end{equation}
where $\set{V}_{\mat{Y}} = \{ 0 \} \cup \left\{ |\set{C}_k|^{-1/2} \right\}_{k=1}^{K}$.
Seeking to apply the desirable properties of SDP to $K$-means, we can pose \citep{Kulis2007,Peng2007_sdk-kmeans}
\begin{equation}
	\max_{\mat{Q} \in \Real^{n \times n}}
	\traceone{\mat{D} \mat{Q}}
	%
	\quad\text{s.t.}\quad
	%
	\begin{aligned}
		& \mat{Q} \vect{1} = \vect{1} , \\	
		& \traceone{\mat{Q}} = K , \\
		& \rank{\mat{Q}} = K , \\
		& \mat{Q} \succeq 0 ,
		\mat{Q} \geq \mat{0} .
	\end{aligned}
	\label[problem]{eq:sdp_kmeans_lowrank}	
\end{equation}
where mixed-integer program is relaxed into the real-valued nonnegative program, directly optimizing over $\mat{Q}$. 
SDP-KM is as a relaxation of this problem, simply obtained by removing the rank constraint.

\section{On the complete positivity of SDP-KM solutions on circulant matrices}
\label{sec:proofs}

% Let $\mat{P}$ be the cyclic permutation matrix, i.e.,
% $\mat{P} =
% 	\left[
% 	\begin{smallmatrix}
% 		\transpose{\vect{0}} & 1 \\
% 		\mat{I} & \vect{0} \\
% 	\end{smallmatrix} \right] $.
% For any circulant matrix $\mat{D}$, we have that $\transpose{\mat{P}} \mat{D} \mat{P} = \mat{D}$ (notice that this implies that $\transpose{\mat{P}^s} \mat{D} \mat{P}^s = \mat{D}$ for any $s \in \Nat$).

% \begin{proposition}
% 	Let $\mat{Q}_*$ be the solution to SDP-KM.
% 	If $\transpose{\mat{P}} \mat{D} \mat{P} = \mat{D}$, then $\transpose{\mat{P}} \mat{Q}_* \mat{P}$ is also the solution to SDP-KM.
% 	Since the problem is convex, $\transpose{\mat{P}} \mat{Q}_* \mat{P} = \mat{Q}_*$, and $\mat{Q}_*$ must be a circulant matrix.
% 	\label{prop:circulant}
% \end{proposition}
% \begin{proof}
% 	We have that for the objective function
% 	\begin{equation}
% 			\traceone{\mat{D} \transpose{\mat{P}} \mat{Q}_* \mat{P}} = \traceone{\mat{P} \mat{D} \transpose{\mat{P}} \mat{Q}_*} = \traceone{\mat{D} \mat{Q}_*}
% 	\end{equation}
% 	and for the constraints, using $\mat{P} \transpose{\mat{P}} = \mat{I}$,
% 	\begin{align}
% 		\traceone{\transpose{\mat{P}} \mat{Q}_* \mat{P}} &= \traceone{\mat{D} \mat{Q}_*} = K , \\
% 		\transpose{\mat{P}} \mat{Q}_* \mat{P} \vect{1} &= \transpose{\mat{P}} \mat{Q}_* \vect{1} = \transpose{\mat{P}} \vect{1} = \vect{1} .
% 	\end{align}
% 	Since $\transpose{\vect{z}} \mat{Q}_* \vect{z} \geq 0$, then $\transpose{\vect{z}} \transpose{\mat{P}} \mat{Q}_* \mat{P} \vect{z} \geq 0$.
% 	Finally, $\mat{Q}_* \geq \mat{0}$ implies that $\transpose{\mat{P}} \mat{Q}_* \mat{P} \geq \mat{0}$.
% \end{proof}

\begin{proposition}
	If the solution $\mat{Q}_*$ to SDP-KM is a circulant matrix,
	then it is CP for every $K \leq 3/2$ or $K \geq \tfrac{n}{2}$.
	\label{prop:circulantCP}%
\end{proposition}

\begin{proof}
	For $K \leq 3/2$, plugging the constraint $\mat{Q}_* \vect{1} = \vect{1}$ into Corollary 2.6 in \citep[][p.~7]{So2013} gives the desired result.
	
	Let us address $K \geq \tfrac{n}{2}$.
	\citet{Kaykobad1987} proved that every diagonally dominant matrix $\mat{A}$, i.e.,
	$|(\mat{A})_{ii}| \geq \sum_{j \neq i} |(\mat{A})_{ij}|$ for all $i$, is a CP matrix.
	We have to prove then that $\mat{Q}_* \geq \mat{0}$ is diagonally dominant.
	We have $\traceone{\mat{Q}_*} = K$ and, since $\mat{Q}_*$ is circulant, all $(\mat{Q}_*)_{ii}$ have the same value. Then, $(\mat{Q}_*)_{ii} = K/n$.
	From $\mat{Q}_* \vect{1} = \vect{1}$,
	$\sum_{j \neq i} (\mat{Q}_*)_{ij} = 1 - (\mat{Q}_*)_{ii} = 1 - K/n$.
	Hence, $\mat{Q}_*$ is diagonally dominant for $K \geq \tfrac{n}{2}$.
\end{proof}

\section{Additional results}
\label{sec:additional_multilayer_results}

We include additional results of the multi-layer NOMAD algorithm using different values of $k$ in each layer.

\begin{figure}
    \includegraphics[width=.618\linewidth]{multilayer/circles-8-4-2}%
    \\[2pt]
    \includegraphics[width=.618\linewidth]{multilayer/circles-12-6-2}%
    \\[2pt]
	\includegraphics[width=.618\linewidth]{multilayer/circles-16-4-2}%
    \\[2pt]
	\includegraphics[width=.744\linewidth]{multilayer/circles-16-8-4-2}%
    \\[2pt]
    \includegraphics[width=\linewidth]{multilayer/circles-16-12-8-6-4-2}%
    \\[2pt]
	\includegraphics[width=.873\linewidth]{multilayer/circles-32-16-8-4-2}%
    \\[2pt]

	\caption{Additional results of multi-layer NOMAD.}
    \label{fig:additional_multilayer_rings}
\end{figure}

\begin{figure}
    \includegraphics[width=.618\linewidth]{multilayer/moons-8-4-2}%
    \\[2pt]
    \includegraphics[width=.618\linewidth]{multilayer/moons-12-6-2}%
    \\[2pt]
	\includegraphics[width=.618\linewidth]{multilayer/moons-16-4-2}%
    \\[2pt]
    \includegraphics[width=\linewidth]{multilayer/moons-16-12-8-6-4-2}%
    \\[2pt]
	\includegraphics[width=.873\linewidth]{multilayer/moons-32-16-8-4-2}%

	\caption{Additional results of multi-layer NOMAD.}
    \label{fig:additional_multilayer_moons}
\end{figure}

\begin{figure}
    \includegraphics[width=.618\linewidth]{multilayer/double_swiss_roll-8-4-2}%
    \\[2pt]
    \includegraphics[width=.618\linewidth]{multilayer/double_swiss_roll-12-6-2}%
    \\[2pt]
	\includegraphics[width=.618\linewidth]{multilayer/double_swiss_roll-16-4-2}%
    \\[2pt]
    \includegraphics[width=\linewidth]{multilayer/double_swiss_roll-16-12-8-6-4-2}%
    \\[2pt]
	\includegraphics[width=.873\linewidth]{multilayer/double_swiss_roll-32-16-8-4-2}%
    \\[2pt]
	\includegraphics[width=.744\linewidth]{multilayer/double_swiss_roll-64-16-4-2}%
    \\[2pt]
	\includegraphics[width=.744\linewidth]{multilayer/double_swiss_roll-64-16-4-2}%
    \\[2pt]
	\includegraphics[width=\linewidth]{multilayer/double_swiss_roll-64-32-16-8-4-2}%

	\caption{Additional results of multi-layer NOMAD.}
    \label{fig:additional_multilayer_double_swiss_roll}
\end{figure}

\section{Symmetric NMF}
\label{sec:snmf}

In this section, we present the algorithm used to compute the symmetric NMF  of a matrix $\mat{A} \in \Real^{n \times n}$, defined as
\begin{equation}
	\min_{\mat{Y} \in \Real^{n \times r}}
	\norm{\mat{A} - \mat{Y} \transpose{\mat{Y}}}{F}^2
	\quad\text{s.t.}\quad
	\mat{Y} \geq \mat{0}.
	%
	\tag{SNMF}
	\label[problem]{eq:snmf}
\end{equation}
We use the alternating direction method of multipliers (ADMM) to solve it.
In short, ADMM solves convex optimization problems by breaking them into smaller subproblems, which are individually easier to handle. It has also been extended to handle non-convex problems, e.g., to solve several flavors of NMF~\citep{Fevotte2011,xu2012nmf,Tepper2014consensus,tepper2016compressed}.

\cref{eq:snmf} can be equivalently re-formulated as
\begin{equation}
	\min_{\mat{Y} \in \Real^{n \times r}}
	\norm{\mat{A} - \mat{Y} \transpose{\mat{X}}}{F}^2
	%
	\quad\text{s.t.}\quad
	%
	\mat{Y} = \mat{X},\
	\mat{Y} \geq \mat{0},\ \mat{X} \geq \mat{0} ,
\end{equation}
and we consider its augmented Lagrangian,
\begin{equation}
	\mathscr{L} \left( \mat{X}, \mat{Y}, \mat{\Gamma} \right) =
	\tfrac{1}{2} \norm{\mat{A} - \mat{Y} \transpose{\mat{X}}}{F}^2
	+ \tfrac{\sigma}{2} \norm{\mat{Y} - \mat{X}}{F}^2
	- \traceone{ \transpose{\mat{\Gamma}} \left( \mat{Y} - \mat{X} \right)}
\end{equation}
where $\mat{\Gamma}$ is a Lagrange multiplier, $\sigma$ is a penalty parameter.

The ADMM algorithm works in a coordinate descent fashion, successively minimizing $\mathscr{L}$ with respect to $\mat{X}, \mat{Y}$, one at a time while fixing the other at its most recent value and then updating the multiplier $\mat{\Gamma}$.
For the problem at hand, these steps are
\begin{subequations}
\begin{align}
	\mat{X}^{(t+1)} &= \argmin_{\mat{X} \geq \mat{0}} \mathcal{L} \left( \mat{X}, \mat{X}^{(t)}, \mat{\Gamma}^{(t)} \right) ,\\
	\mat{Y}^{(t+1)} &= \argmin_{\mat{Y} \geq \mat{0}} \mathcal{L} \left( \mat{X}^{(t+1)}, \mat{Y}, \mat{\Gamma}^{(t)} \right) ,\\
	\mat{\Gamma}^{(t+1)} &= \mat{\Gamma}^{(t)} - \eta \sigma \left( \mat{X}^{(t+1)} - \mat{Y}^{(t+1)} \right) .
\end{align}
\end{subequations}
In our experiments, we fix $\eta$ and $\sigma$ to 1. We initialize the algorithm with a random matrix.

\section{Non-convex SDP solver}
\label{sec:burer-monteiro}

We follow the algorithm proposed in \cite{Kulis2007,Hou2015} to solve \cref{eq:sdp_kmeans_lowrank_fast}. Our approach has a small but fundamental difference: instead of setting $r = K$, we allow for $r \geq K$.
We define the augmented Lagrangian of \cref{eq:sdp_kmeans_lowrank_fast} as
\begin{equation}
	\begin{aligned}
		\mathcal{L} \left( \mat{Y}, \vect{\mu}, \lambda \right) =
		& -\traceone{\mat{D} \transpose{\mat{Y}} \mat{Y}}
		+ \tfrac{\sigma}{2} \norm{\transpose{\mat{Y}} \mat{Y} \vect{1} - \vect{1}}{2}^2
		- \transpose{\vect{\mu}} (\transpose{\mat{Y}} \mat{Y} \vect{1} - \vect{1}) \\
		& + \tfrac{\varphi}{2} (\traceone{\transpose{\mat{Y}} \mat{Y}} - K)^2
		- \vect{\lambda} (\traceone{\transpose{\mat{Y}} \mat{Y}} - K) ,
	\end{aligned}
\end{equation}
where $\vect{\mu}, \vect{\lambda}$ are Lagrange multipliers, $\sigma, \varphi$ are penalty parameters.
We obtain $\mat{Y}$ by running the steps
\begin{subequations}
\begin{align}
	\mat{Y}^{(t+1)} &= \argmin_{\mat{Y} \geq \mat{0}} \mathcal{L} \left( \mat{Y}, \vect{\mu}^{(t)}, \lambda^{(t)} \right) ,\\
	\vect{\mu}^{(t+1)} &= \vect{\mu}^{(t)} - \eta \sigma \left( \transpose{\mat{Y}} \mat{Y} \vect{1} - \vect{1} \right) ,\\
	\lambda^{(t+1)} &= \lambda^{(t)} - \eta \varphi \left( \traceone{\transpose{\mat{Y}} \mat{Y}} - K \right) .
\end{align}
\end{subequations}
This is a non-standard approach since the minimization over $\mat{Y}$ (the gradient $\partial \mathcal{L} / \partial \mat{Y}$ is given in \cite{Hou2015}) is a non-convex problem.
Although there are no guarantees about the convergence of the procedure, theoretical assurances for related problems have been presented in \cite{boumal2016non}.
To perform the minimization with respect to $\mat{Y}$, we use the L-BFGS-B algorithm \citep{Byrd1995} with bound constraints ($(\mat{Y})_{ij} \in [0, 1]$). Finally, the initialization to the overall iterative algorithm is done with symmetric nonnegative matrix factorization, see \cref{sec:snmf}.
In our experiments, we fix $\eta$, $\varphi$, and $\sigma$ to 1 and prenormalize $\mat{D}$ (dividing by its Frobenius norm).

\section{Proofs for the conditional gradient algorithm}
\label{sec:cgm_proofs}

This section closely follows the works of \citet{Hazan2008sdp} and \citet{Clarkson2010fw}.

\begin{lemma}
	The dual objective of
    \begin{equation}
		\max_{\mat{Z}}
    	f(\mat{Z})
    	%
		\quad\text{s.t.}\quad
		%
    	\mat{Z} \vect{b} = \vect{0} ,
    	\quad
		\traceone{\mat{Z}} = k - 1 ,
   		\quad
		\mat{Z} \succeq \mat{0}
		%
	\end{equation}
    is
    \begin{equation}
    	\min_{\mat{Z}} w(\mat{Z}) ,
    \end{equation}    
    where
    \begin{align}
    	w(\mat{Z}) &= s \, \phi(\mat{Z}) + f(\mat{Z}) - \traceone{\mat{Z} \nabla f(\mat{Z})} ,
        \label{eq:generic_sdp_ortho_dual_w} \\
    	\phi(\mat{Z}) &=
        \max_{\substack{
            \norm{\vect{v}}{2} = 1\\
            \transpose{\vect{v}} \vect{b} = 0
        }}
        \transpose{\vect{v}} \nabla f(\mat{Z}) \vect{v} .
        \label{eq:generic_sdp_ortho_dual_phi}
    \end{align}
    \label[lemma]{thm:generic_sdp_ortho_dual}
\end{lemma}

\proof{
	The Lagrangian relaxation of \cref{eq:generic_sdp_ortho} is
    \begin{equation}
    \begin{aligned}
    	\ell = -\max_{\mat{\Psi}, \psi, \vect{y}}
        \min_{\mat{Z}}
        &\ -f(\mat{Z}) - \traceone{\mat{\Psi} \mat{Z}} \\
        &+ \psi (\traceone{\mat{Z}} - s) + \transpose{\vect{y}} \mat{Z} \vect{b} ,
        \label{eq:generic_sdp_ortho_lagrangian}
    \end{aligned}
    \end{equation}
    where $\mat{\Psi} \succeq \mat{0}$, $\psi \in \Real$, and $\vect{y} \in \Real^n$ are Lagrange multipliers.
    Differentiating and equating to zero we get
    $\mat{\Psi} = -\nabla f(\mat{Z}) + \psi \mat{I} + \vect{y} \transpose{\vect{b}}$.
    Note that $\mat{\Psi} \succeq \mat{0}$ implies that $\vect{y} = c \vect{b}$ for some $c \in \Real$, yielding
    \begin{equation}
    	\mat{\Psi} = -\nabla f(\mat{Z}) + \psi \mat{I} + c \vect{b} \transpose{\vect{b}} \succeq \mat{0} .
        \label{eq:generic_sdp_ortho_U}
    \end{equation}    
    Plugging \cref{eq:generic_sdp_ortho_U} and $\vect{y} = c \vect{b}$ in \cref{eq:generic_sdp_ortho_lagrangian} we get 
    \begin{align}
    	\phantom{\ell}
        &\begin{aligned}
    		\mathllap{\ell}
        	=
			\max_{\psi}
          \min_{\mat{Z}}
          \ &f(\mat{Z}) - \traceone{\left( \nabla f(\mat{Z}) + \psi \mat{I} + c \vect{b} \transpose{\vect{b}} \right) \mat{Z}} \\
          &+ \psi (\traceone{\mat{Z}} - s) + c \transpose{\vect{b}} \mat{Z} \vect{b} \\
        \end{aligned}
        \\
        %
        &= \max_{\psi \in \Real}
        \min_{\mat{Z}}
        f(\mat{Z}) - \traceone{\nabla f(\mat{Z}) \ \mat{Z}} + \psi s \\
        %
        &= \max_{\substack{
        	\mat{Z} \\
            \psi \in \Real
        }}
        f(\mat{Z}) - \traceone{\nabla f(\mat{Z}) \ \mat{Z}} - \psi s .
    \end{align}
    %where the last equality amounts to noticing that under the constraint in \cref{eq:generic_sdp_ortho_U}, $\mat{Z}$ is uniquely determined.
    
    From \cref{eq:generic_sdp_ortho_U}, $\psi \mat{I} \succeq \nabla f(\mat{Z}) - c \vect{b} \transpose{\vect{b}}$, implying
    \begin{subequations}
    \begin{align}
    	 \psi
         &\geq \lambda_{\text{max}} \left\{ \nabla f(\mat{Z}) - c \vect{b} \transpose{\vect{b}} \right\} \\
         &\geq \lambda_{\text{max}} \left\{ \nabla f(\mat{Z}) - d \vect{b} \transpose{\vect{b}} \right\}
         \quad \forall d > c \\
         &\geq \phi(\mat{Z}).
    \end{align}    
    \end{subequations}
    The last inequality comes from taking $d \rightarrow +\infty$, thus shifting the eigenvalue associated with $\vect{b}$ (should there be one) away from the maximum.
    Without loss of generality, we set $\psi = \phi(\mat{Z})$, finally obtaining $\ell = \min_{\mat{Z}} w(\mat{Z})$.
}

\begin{proposition}
Let $\mat{X}, \mat{Z} \in \set{P}_s$ and $\mat{Y} = \mat{X} + \alpha (\mat{Z} - \mat{X})$ and $\alpha \in \Real$.
    The curvature constant of $f$ is
	\begin{equation}
	C_f \defeq
    \sup_{\mat{X}, \mat{Z}, \alpha}
    \tfrac{1}{\alpha^2}
        [ f(\mat{X}) - f(\mat{Y}) + \tracetwo{(\mat{Y} - \mat{X})}{\nabla f(\mat{X})} ] .
        %
	\end{equation}    
	Let $\mat{Z}^{\star}$ be the solution to 
    \begin{equation}
		\max_{\mat{Z}}
    	f(\mat{Z})
    	%
		\quad\text{s.t.}\quad
		%
    	\mat{Z} \vect{b} = \vect{0} ,
    	\quad
		\traceone{\mat{Z}} = k - 1 ,
   		\quad
		\mat{Z} \succeq \mat{0} .
		%
	\end{equation}
	The iterates $\mat{Z}_t$ of \cref{algo:cgm_generic_sdp_ortho} satisfy for all $t > 1$
    \begin{equation}
    	f(\mat{Z}^{\star}) - f(\mat{Z}_t) \leq  \tfrac{8 C_f}{t+2} .
    \end{equation}
\end{proposition}

\proof{
    Let
    \begin{equation}
    	h(\mat{Z}) = \tfrac{1}{4 C_f} [ f(\mat{Z}^{\star}) - f(\mat{Z}) ] .
    \end{equation}
    Proving that $h(\mat{Z}_{t}) \leq \tfrac{2}{t + 2}$ yields the desired result.
	From \cref{thm:generic_sdp_ortho_dual}, we have
    \begin{equation}
    	w(\mat{Z}) \geq w(\mat{Z}^{\star}) \geq f(\mat{Z}^{\star}) \geq f(\mat{Z}) .
        %
        \label{eq:weak_duality}
    \end{equation}
	By \cref{eq:generic_sdp_ortho_dual_w,eq:generic_sdp_ortho_dual_phi}, we have
    \begin{align}
    	\transpose{\vect{v}}_t \nabla f(\mat{Z}_t) \vect{v}_t
        &= \phi(\mat{Z}) \\
        &= w(\mat{Z}_t) - f(\mat{Z}_t) + \traceone{\mat{Z} \ \nabla f(\mat{Z}_t)} .
    \end{align}
    Therefore,
    \begin{equation}
    	\traceone{(\mat{H}_t - \mat{Z}_t) \ \nabla f(\mat{Z}_t)} = w(\mat{Z}_t) - f(\mat{Z}_t) .
        \label{eq:w_minus_f}
    \end{equation}
    Now, using \cref{eq:curvature_constant}
    \begin{subequations}
    \begin{align}
    	f(\mat{Z}_{t+1})
        &= f(\mat{Z}_{t} + \alpha_t ( \mat{H}_t - \mat{Z}_{t} ) ) \\
        %
        &\geq f(\mat{Z}_{t}) + \alpha_t \traceone{( \mat{H}_t - \mat{Z}_{t}) \ \nabla f(\mat{Z}_t) } + \alpha^2 C_f .
        \label{eq:f_inequality1}
    \end{align}
    \end{subequations}    
    Putting \cref{eq:f_inequality1} together with \cref{eq:weak_duality,eq:w_minus_f},
    \begin{subequations}
    \begin{align}
    	f(\mat{Z}_{t+1})
        &\geq f(\mat{Z}_{t}) + \alpha_t ( w(\mat{Z}_t) - f(\mat{Z}_t) ) - \alpha_t^2 C_f \\
        %
        &\geq f(\mat{Z}_{t}) + \alpha_t ( f(\mat{Z}^{\star}) - f(\mat{Z}_t) ) - \alpha_t^2 C_f \\
        %
%         &= f(\mat{Z}_{t}) + 4 \alpha_t C_f g(\mat{Z}_{t}) - \alpha_t^2 C_f \\
        &= f(\mat{Z}_{t}) + 4 \alpha_t C_f h(\mat{Z}_{t}) - \alpha_t^2 C_f .
        %
        \label{eq:f_inequality}
    \end{align}
    \end{subequations}
    From the definition of $h(\mat{Z}_{t})$, this implies
    \begin{equation}
    	h(\mat{Z}_{t+1}) \leq h(\mat{Z}_{t}) - \alpha_t h(\mat{Z}_{t}) + \tfrac{\alpha_t^2}{4} .
    \end{equation}
%     Let $\epsilon_t = \tfrac{C_f}{t^2} \geq C_f h(\mat{Z}_{t})$; by this choice,
%     \begin{equation}
%     	h(\mat{Z}_{t+1}) \geq h(\mat{Z}_{t}) - \alpha_t h(\mat{Z}_{t}) + \tfrac{\alpha_t^2}{2}.
%     \end{equation}
    Finally, we prove inductively that $h(\mat{Z}_{t}) \leq \tfrac{2}{t + 2}$. In the first iteration, $\alpha_1 = 1$ and $h(\mat{Z}_{2}) \leq \tfrac{1}{4}$. By taking $\alpha = \tfrac{2}{t + 2}$, we have
    \begin{subequations}
    \begin{align}
    	h(\mat{Z}_{t+1})
        &\leq h(\mat{Z}_{t}) - \alpha_t h(\mat{Z}_{t}) + \tfrac{\alpha_t^2}{4} \\
        &\leq (1 - \alpha_t) h(\mat{Z}_{t}) + \tfrac{\alpha_t^2}{2} \\
        &= (1 - \tfrac{2}{t + 2}) \tfrac{2}{t + 2} + \tfrac{2}{(t + 2)^2} \leq \tfrac{2}{t + 3} .
    \end{align}
    \end{subequations}
}

